Initial performance studies of a general-purpose detector for multi-TeV physics at a 100 TeV pp collider

This paper describes simulations of detector response to multi-TeV physics at the Future Circular Collider (FCC-hh) or Super proton-proton Collider (SppC) which aim to collide proton beams with a centre-of-mass energy of 100 TeV. The unprecedented energy regime of these future experiments imposes new requirements on detector technologies which can be studied using the detailed GEANT4 simulations presented in this paper. The initial performance of a detector designed for physics studies at the FCC-hh or SppC experiments is described with an emphasis on measurements of single particles up to 33 TeV in transverse momentum. The reconstruction of hadronic jets has also been studied in the transverse momentum range from 50 GeV to 26 TeV. The granularity requirements for calorimetry are investigated using the two-particle spatial resolution achieved for hadron showers.

==> Makefile <==
###############################################################################
#
# Makefile for the photon note
#                              	
###############################################################################

NOTENAME=sifcc


all:#default target makes everything
	latex $(NOTENAME).tex && bibtex $(NOTENAME) && latex $(NOTENAME).tex && latex $(NOTENAME).tex && dvips -Ppdf -G0 $(NOTENAME).dvi && ps2pdf $(NOTENAME).ps

show:
	ps2pdf $(NOTENAME).ps && evince $(NOTENAME).pdf

.PHONY: clean
clean:
	rm -rf $(NOTENAME).aux $(NOTENAME).log $(NOTENAME).dvi $(NOTENAME).out $(NOTENAME).bbl $(NOTENAME).blg\
	$(NOTENAME).dvi $(NOTENAME).ps \
	$(NOTENAME).toc $(NOTENAME).tof thumb*.* *~ 
	rm $(NOTENAME).pdf

